Automated Requirements Relation Extraction

In the context of requirements engineering, relation extraction involves identifying and documenting the associations between different requirements artefacts. When dealing with textual requirements (i.e., requirements expressed using natural language), relation extraction becomes a cognitively challenging task, especially in terms of ambiguity and required effort from domain-experts. Hence, in highly-adaptive, large-scale environments, effective and efficient automated relation extraction using natural language processing techniques becomes essential. In this chapter, we present a comprehensive overview of natural language-based relation extraction from text-based requirements. We initially describe the fundamentals of requirements relations based on the most relevant literature in the field, including the most common requirements relations types. The core of the chapter is composed by two main sections: (i) natural language techniques for the identification and categorization of equirements relations (i.e., syntactic vs. semantic techniques), and (ii) information extraction methods for the task of relation extraction (i.e., retrieval-based vs. machine learning-based methods). We complement this analysis with the state-of-the-art challenges and the envisioned future research directions. Overall, this chapter aims at providing a clear perspective on the theoretical and practical fundamentals in the field of natural language-based relation extraction.

==> contents/DUMP_05_evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

In this section, we outline the evaluation metrics for assessing the performance of relation extraction methods in the context of natural language processing for requirements engineering. We align the evaluation criteria with ISO/IEC 25010~\cite{ISO25010}, which provides a vocabulary for software product quality.

\subsection{Quality characteristics}

ISO 25010 defines two key aspects relevant to the evaluation of relation extraction tasks:

\begin{itemize}
\item \textbf{Functional Suitability:} The degree to which the product or system provides functions that meet stated and implied needs when used under specified conditions. Relation extraction mainly focuses on two sub-characteristics. \textit{Functional correctness} addresses the accuracy of the extracted relations, particularly for binary or multi-class classification tasks. For binary relation extraction, we mainly measure positive (relation exists) and negative (no relation) predictions. For multi-class extraction, we identify different types of positive predictions (e.g., requires, conflicts, duplicates, exemplifies, contradicts), as well as negative predictions (no relation). On the other hand, \textit{functional appropriateness} focuses on whether the extracted relations are relevant and meaningful in the context of requirements engineering. While automated evaluation metrics are commonly used for functional correctness, assessing functional appropriateness may require human judgment.

\item \textbf{Performance Efficiency:} The performance relative to the amount of resources used under stated conditions. Relation extraction typically focuses on \textit{time behaviour}, a sub-characteristic that pertains to the efficiency and timeliness of the extraction process. It focuses on how well the relation extraction method performs concerning the speed of identifying and processing relations within a given set of textual requirements.
\end{itemize}

\subsection{Functional suitability: methods and metrics}

\subsubsection{Functional correctness.} The evaluation methods for functional correctness include:

\begin{itemize}
\item \textbf{Binary or Multi-class Classification Matrix:} A confusion matrix for binary or multi-class classification represents true positive (TP), true negative (TN), false positive (FP), and false negative (FN) predictions. For binary classification, TP identifies true relations, TN recognizes true non-relations, FP indicates false relations, and FN signifies missed relations. %TP refers to correctly identifying the presence of a relation between two requirements, TN represents correctly recognizing the absence of a relation, FP indicates wrongly predicting the presence of a relation, and FN denotes wrongly predicting the absence of a relation. 
For multi-class classification, the confusion matrix extends to multiple classes (relation types), where each cell of the matrix corresponds to the correct and incorrect predictions for each relation type.

\item \textbf{Precision:} Measures the accuracy of positive relation predictions. It is the ratio of correctly predicted positive relations to the total number of relations predicted as positive.

\item \textbf{Recall:} Assesses the ability of the method to identify all positive relations correctly. It is the ratio of correctly predicted positive relations to the total number of actual positive relations in the dataset.

\item \textbf{F-measure:} Balanced metric that combines precision and recall for relation extraction tasks. It represents the harmonic mean of precision and recall, providing an overall measure of the method's performance in identifying positive relations accurately.

\item \textbf{Accuracy:} Refers to the ratio of correctly predicted relations (both positive and negative) to the total number of relations in the dataset. It evaluates the overall correctness of the extraction method in identifying all types of relations.

\item \textbf{Mean Average Precision (mAP):} Calculated by averaging the precision scores at different recall levels~\cite{Shin2015}. It provides a single value that allows comparison across different datasets, reflecting the method's ability to rank and retrieve relevant relations effectively. Average precision (AP) is defined as follows:

\begin{equation}
    AP = \sum_n (R_n - R_{n-1}) P_n \text{,}
\end{equation}

where $R_n$ and $P_n$ are precision and recall at the $n$th position, respectively. Consequently, mAP is defined as follows:

\begin{equation}
    mAP = \frac{1}{n}\sum_{i=1}^{n}(AP_i) \text{,}
\end{equation}

where $n$ is the number of classes (i.e., the number of relation types, including the non-related prediction) and $AP_i$ is the average precision for class $i$.

%\item \textbf{Lag:} Measures the positioning of correct links within the ranked list of extracted relations~\cite{Shin2015}. It quantifies how many incorrect links are retrieved above each correct link in the list, and it is defined as follows:

%\begin{equation}
%    Lag = \frac{1}{RR_T} \sum_{(r_i, r_j) \in RR_T} Lag((r_i, r_j)) \text{,}
%\end{equation}

%where $RR_T$ is the set of correctly predicted relations and $Lag(r_i, r_j)$ is the amount of incorrect predicted relations with a confidence score higher than some correct prediction $(r_i, r_j)$.

%\item \textbf{Area Under the ROC curve (AUC):} Area under a Receiver Operating Characteristic (ROC) curve~\cite{Shin2015}. Each point on the ROC curve corresponds to a pair of values representing recall and False Positive (FP) rate, respectively. AUC measures how effectively the relation extraction technique differentiates between relevant and non-relevant relations.

\end{itemize}

\subsubsection{Functional appropriateness.} The evaluation methods for functional appropriateness include:

\begin{itemize}
\item \textbf{Kappa Agreement:} A statistical measure to assess the agreement between multiple human annotators when assigning relation types, helping to determine the consistency and quality of the extracted relations.
\item \textbf{Questionnaires/Interviews:} Involving domain experts to review and assess the relevance and appropriateness of the extracted relations. The feedback obtained through questionnaires and interviews helps to evaluate how well the relation extraction method aligns with the specific needs and requirements of the users, and whether the extracted relations are meaningful and useful for the intended use case. Beyond the quality of the predictions, experts might also provide insights on complementary details on context-specific scenarios, including the importance of early detection, the impact of reporting false positives with respect to missing undetected relations and the formalization of types of dependencies.
\end{itemize}

\subsection{Performance efficiency: methods and metrics}

\subsubsection{Execution time.} This aspect measures the time taken by the relation extraction method to process a given set of requirements and identify the relations. To evaluate performance efficiency, we compare the execution time of the method with manual efforts or other baseline approaches (e.g., manual relation extraction, domain expert ontology design), assessing the scalability and practicality of the solution.

While execution time is widely extended for measuring the quality of extraction methods, it is difficult to find references to other performance efficiency metrics (e.g., resource utilization) in the context of requirement relation extraction. 

\begin{tcolorbox}
[width=\linewidth, sharp corners=all, colback=white!95!black, boxrule=0.2pt, boxsep=1pt,left=2pt,right=2pt,top=2pt,bottom=2pt]
\includegraphics[height=10pt]{figures/colab.png}
Read and execute \textit{Section 7. Evaluation} from the Jupyter Notebook for an exemplified illustration of functional suitability and performance efficiency metrics in the context of a multi-class relation extraction, machine learning-based task with the PURE dataset.
\end{tcolorbox} 

%By using these evaluation metrics, researchers and practitioners can effectively assess the quality and efficiency of relation extraction methods, facilitating the advancement of natural language processing techniques for requirements engineering tasks.
